From Local to Global: Sheaf-Theoretic Control Barrier Functions on Manifolds

Control barrier functions (CBFs) provide formal safety guarantees for dynamical systems by rendering a safe set forward-invariant via pointwise-optimal feedback control. While the CBF framework is well established for dynamical systems in Euclidean space, there exist gaps for systems evolving on non-Euclidean manifolds. For systems modeled as constrained control differential inclusions, we introduce the Sheaf-CBF: a sheaf-theoretic framework for CBFs on smooth manifolds and vector bundles. The differential inclusions are formulated intrinsically on the control bundle, and analogous regularity properties in the Euclidean case are established fiberwise under local trivializations. Regularity conditions are given under which a pointwise-optimal feedback law is single-valued and continuous over local charts. Framed as a local-to-global optimization problem, sheaf-theoretic restriction and gluing compatibility conditions on overlapping charts are shown to uniquely determine a continuous global section of the control bundle, thereby guaranteeing forward invariance of the safe set. Numerical simulations on a nontrivial M{\"o}bius strip demonstrate that failure of sheaf compatibility results in violations of safety, whereas the Sheaf-CBF maintains forward invariance.

==> preamble.tex <==
%% ======== CORE MATH PACKAGES ========= %%
\usepackage{amsmath}     % Core math
\usepackage{amssymb}     % Math symbols
\usepackage{amsfonts}    % Additional math fonts
\usepackage{mathtools}   % Math extensions
\usepackage{enumitem}

%% ======== THEOREM ENVIRONMENTS ======= %%
\usepackage{amsthm}

% Numbered theorems within sections
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture} % <-- added


% Definitions and examples in roman font
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{example}[theorem]{Example}
\newtheorem{assumption}[theorem]{Assumption} % <-- added

% Remarks in italic (default)
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{note}[theorem]{Note}

%% ======== DIAGRAMS =================== %%
\usepackage{tikz-cd}     % Category-theoretic diagrams
\usepackage{quiver}      % Flexible categorical diagrams
\usepackage{tikz}
\usetikzlibrary{calc,decorations.pathreplacing}
\usetikzlibrary{arrows.meta,decorations.pathreplacing}
\usetikzlibrary{animations} % LaTeX and plain TeX
\usetikzlibrary[animations] % ConTeXt

%% ======== TODOS AND ANNOTATIONS ====== %%
\usepackage{todonotes}
\todostyle{keith}{color=purple!40,inline,author=KC}
\todostyle{brandon}{color=pink!40,inline,author=BF}
\todostyle{wilmer}{color=green!40,inline,author=WL}
\todostyle{any}{color=red!30,inline,author=ANY}

%% ======== CUSTOM MATH MACROS ========= %%
% Categories and general notation
\newcommand{\cat}[1]{\mathsf{#1}}
\newcommand{\Sub}{\cat{Sub}}
\newcommand{\SubKop}{\cat{Sub \circ K^{op}}}
\newcommand{\SubPosK}{\cat{SubPosK}}
\newcommand{\Dynam}{\cat{Dynam}}
\newcommand{\FinSet}{\cat{FinSet}}
\newcommand{\Vect}{\cat{Vect}}
\newcommand{\Graph}{\cat{Graph}}
\newcommand{\Pos}{\cat{Pos}}
\newcommand{\Set}{\cat{Set}}
\newcommand{\decomp}{\cat{Dcmp}}



% Others
\newcommand{\R}{\mathbb{R}}

% Custom morphism symbol
\def\tobar{\mathrel{\mkern3mu  \vcenter{\hbox{$\scriptscriptstyle+$}}%
                    \mkern-12mu{\to}}}

%% ======== UTILITY ==================== %%
\usepackage{comment}     % Enables \begin{comment}...\end{comment}

%% ======== DOUBLESTRUCK & CALIGRAPHIC == %%
% (your \DeclareMathOperator block remains unchanged)
\DeclareMathOperator{\Aa}{\mathcal{A}}  \DeclareMathOperator{\Ab}{\mathbb{A}}
\DeclareMathOperator{\Ba}{\mathcal{B}}  \DeclareMathOperator{\Bb}{\mathbb{B}}
\DeclareMathOperator{\Ca}{\mathcal{C}}  \DeclareMathOperator{\Cb}{\mathbb{C}}
\DeclareMathOperator{\Da}{\mathcal{D}}  \DeclareMathOperator{\Db}{\mathbb{D}}
\DeclareMathOperator{\Ea}{\mathcal{E}}  \DeclareMathOperator{\Eb}{\mathbb{E}}
\DeclareMathOperator{\Fa}{\mathcal{F}}  \DeclareMathOperator{\Fb}{\mathbb{F}}
\DeclareMathOperator{\Ga}{\mathcal{G}}  \DeclareMathOperator{\Gb}{\mathbb{G}}
\DeclareMathOperator{\Ha}{\mathcal{H}}  \DeclareMathOperator{\Hb}{\mathbb{H}}
\DeclareMathOperator{\Ia}{\mathcal{I}}  
\DeclareMathOperator{\Ja}{\mathcal{J}}  
\DeclareMathOperator{\Ka}{\mathcal{K}}  \DeclareMathOperator{\Kb}{\mathbb{K}}
\DeclareMathOperator{\La}{\mathcal{L}}  \DeclareMathOperator{\Lb}{\mathbb{L}}
\DeclareMathOperator{\Ma}{\mathcal{M}}  \DeclareMathOperator{\Mb}{\mathbb{M}}
\DeclareMathOperator{\Na}{\mathcal{N}}  \DeclareMathOperator{\Nb}{\mathbb{N}}
\DeclareMathOperator{\Oa}{\mathcal{O}}  \DeclareMathOperator{\Ob}{\mathbb{O}}
\DeclareMathOperator{\Pa}{\mathcal{P}}  \DeclareMathOperator{\Pb}{\mathbb{P}}
\DeclareMathOperator{\Qa}{\mathcal{Q}}  \DeclareMathOperator{\Qb}{\mathbb{Q}}
\DeclareMathOperator{\Ra}{\mathcal{R}}  \DeclareMathOperator{\Rb}{\mathbb{R}}
\DeclareMathOperator{\Sa}{\mathcal{S}}  \DeclareMathOperator{\Sb}{\mathbb{S}}
\DeclareMathOperator{\Ta}{\mathcal{T}}  \DeclareMathOperator{\Tb}{\mathbb{T}}
\DeclareMathOperator{\Ua}{\mathcal{U}}  \DeclareMathOperator{\Ub}{\mathbb{U}}
\DeclareMathOperator{\Va}{\mathcal{V}}  \DeclareMathOperator{\Vb}{\mathbb{V}}
\DeclareMathOperator{\Wa}{\mathcal{W}}  \DeclareMathOperator{\Wb}{\mathbb{W}}
\DeclareMathOperator{\Xa}{\mathcal{X}}  \DeclareMathOperator{\Xb}{\mathbb{X}}
\DeclareMathOperator{\Ya}{\mathcal{Y}}  \DeclareMathOperator{\Yb}{\mathbb{Y}}
\DeclareMathOperator{\Za}{\mathcal{Z}}  \DeclareMathOperator{\Zb}{\mathbb{Z}}
\DeclareMathOperator{\supp}{supp}

% Basic operators
\DeclareMathOperator{\vect}{vec}        % vectorization operator
\DeclareMathOperator{\interior}{int}    % interior of a set
\DeclareMathOperator{\boundary}{\partial} % boundary of a set
\DeclareMathOperator{\neigh}{\mathcal{N}} % neighborhood
\DeclareMathOperator{\id}{Id}           % identity operator

% Additional set and topology operators
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\cod}{cod}
\DeclareMathOperator{\img}{Im}
\DeclareMathOperator{\cl}{cl}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\aff}{aff}

% Differential and geometric operators
\DeclareMathOperator{\grad}{\nabla}
\DeclareMathOperator{\Div}{div}
\DeclareMathOperator{\Lap}{\Delta}
\DeclareMathOperator{\Lie}{L}           % Lie derivative

% Clarke generalized operators
\newcommand{\Clarke}{\partial}
\newcommand{\ClDir}[2]{#1^\circ(#2)}

% Common spaces
\newcommand{\Rn}{\mathbb{R}^n}
\newcommand{\Rm}{\mathbb{R}^m}
\newcommand{\Rnm}{\mathbb{R}^{n\times m}}

% Index set
\newcommand{\ints}[1]{\left[#1\right]}

% Safe set notation
\newcommand{\Safe}{\mathcal{S}}
\newcommand{\Obs}{\mathcal{O}}
\newcommand{\G}{\mathcal{G}}

% Vector and matrix boldface shortcuts
\newcommand{\vx}{\mathbf{x}}
\newcommand{\vy}{\mathbf{y}}
\newcommand{\vu}{\mathbf{u}}
\newcommand{\va}{\mathbf{a}}
\newcommand{\vb}{\mathbf{b}}
\newcommand{\vzero}{\mathbf{0}}

\newcommand{\mA}{\mathbf{A}}
\newcommand{\mI}{\mathbf{I}}

% Column-stacking operator
\newcommand{\col}{\operatorname{col}}


%% ======== ALGORITHMS ================= %%
\usepackage{algorithm}
\usepackage[noend]{algorithmic}

%% ======== TABLES & LINKS ============= %%
\usepackage{tabularx}
\usepackage[colorlinks=true,linkcolor=blue,citecolor=blue,urlcolor=blue]{hyperref}

